Increasing Adversarial Uncertainty to Scale Private Similarity Testing

Social media and other platforms rely on automated detection of abusive content to help combat disinformation, harassment, and abuse. One common approach is to check user content for similarity against a server-side database of problematic items. However, this method fundamentally endangers user privacy. Instead, we target client-side detection, notifying only the users when such matches occur to warn them against abusive content. Our solution is based on privacy-preserving similarity testing. Existing approaches rely on expensive cryptographic protocols that do not scale well to large databases and may sacrifice the correctness of the matching. To contend with this challenge, we propose and formalize the concept of similarity-based bucketization~(SBB). With SBB, a client reveals a small amount of information to a database-holding server so that it can generate a bucket of potentially similar items. The bucket is small enough for efficient application of privacy-preserving protocols for similarity. To analyze the privacy risk of the revealed information, we introduce a framework for measuring an adversary's confidence in inferring a predicate about the client input correctly. We develop a practical SBB protocol for image content, and evaluate its client privacy guarantee with real-world social media data. We then combine SBB with various similarity protocols, showing that the combination with SBB provides a speedup of at least 29x on large-scale databases compared to that without, while retaining correctness of over 95%.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> latexpand <==
#!/usr/bin/perl
# Inspired by latexpand by D. Musliner, University of Michigan
# 2012-2019: Matthieu Moy <git@matthieu-moy.fr>
# BSD License

use strict;
use Cwd;
use Getopt::Long;
use IO::Handle;
use File::Spec;

my $TEXINPUTS = $ENV{'TEXINPUTS'};
# By default, search in current directory. We use '.' and not getcwd()
# to avoid issues if the working directory contains a ':' character.
if (!$TEXINPUTS) { $TEXINPUTS = '.'; }

my $verbose;
my $keep_comments;
my $keep_includes;
my $empty_comments;
my $help;
my $long_help;
my $output;
my $explain;
my $show_graphics;
my $graphics_extensions = ":.pdf:.png:.jpg:.eps";
my $expand_usepackage;
my $expand_bbl;
my $biber;
my $fatal;
my $version;
my $makeatletter;
my $inside_import;
my $in_enc = "bytes";
my $out_enc = "bytes";

GetOptions (
	'h' => \$help,
	'help' => \$long_help,
	'verbose|v' => \$verbose,
	'keep-comments' => \$keep_comments,
	'keep-includes' => \$keep_includes,
	'empty-comments' => \$empty_comments,
	'output|o=s' => \$output,
	'explain' => \$explain,
	'show-graphics' => \$show_graphics,
	'graphics-extensions' => \$graphics_extensions,
	'expand-usepackage' => \$expand_usepackage,
	'expand-bbl=s' => \$expand_bbl,
	'biber=s' => \$biber,
	'fatal' => \$fatal,
	'version' => \$version,
        'makeatletter' => \$makeatletter,
	'in-encoding=s' => \$in_enc,
	'out-encoding=s' => \$out_enc,
) or pod2usage_wrapper(2);
version() if $version;
pod2usage_wrapper(0) if $help;
pod2usage_wrapper(-exitstatus => 0, -output => \*STDOUT, -verbose => 2) if $long_help;

sub pod2usage_wrapper
{
	# Like pod2usage, but fall back to a simpler implem in case
	# pod2usage can't be found.
	if  (eval {require Pod::Usage;1;} ne 1) {
		print "Please install perldoc and Pod::Usage to get proper help.\n";
		my $started = 0;
		open (my $in, '<', "$0") or die $!;
		while (<$in>) {
			if ($started) {
				print;
			}
			if (/^__END__$/) {
				$started = 1;
			}
		}
	} else {
		Pod::Usage->import();
		pod2usage(@_);
	}
}

sub get_version
{
	# $VERSION's value will be substituted by 'make dist', but the
	# next line won't (the string has to be broken to avoid it).
	my $VERSION = 'v1.6';
	if ($VERSION eq '@LATEXPAND' . '_VERSION@') {
		my($vol,$dir,$file) = File::Spec->splitpath($0);
		chdir($dir);
		$VERSION = `git describe --tags HEAD 2>/dev/null`;
	}
	if ($VERSION eq '') {
		$VERSION = '<unknown version>';
	}
	$VERSION =~ s/^\s+|\s+$//g;
	return $VERSION;
}

sub version
{
	print "latexpand version ". get_version() .".\n";
	exit(0);
}

my $nl = "";
if ($empty_comments) {
	$nl = "%\n";
}

if ($output && $output ne "-") {
	open (my $OUTPUT, '>', "$output") or die $!;
	STDOUT->fdopen(\*$OUTPUT, 'w') or die $!;
}

sub say
{
	if ($verbose) {
		print STDERR "$_[0]";
	}
}

my $makeatletter_found;
my $in_preamble;

use open IN  => ":$in_enc", OUT => ":$out_enc";

foreach my $file (@ARGV)
{
	say "processing $file\n";
	$makeatletter_found = 0;
	$in_preamble = 1;
        $inside_import = "";
	process_file($file, "  ");
}

sub cat_file
{
	my $file = shift;
	open (my $INFILE, "<", $file) || die "could not open input file '$file'\n";
	while (<$INFILE>) {
		print;
	}
	close ($INFILE);
}

sub process_file
{
	my $file = shift;
	my $prefix = (shift || "");
	my $in_comment = 0;
	open(my $FILE, "<", $file) or die "could not open input file '$file'\n";
	my $commented_newline = 0;
	while (my $line = <$FILE>) {
		if ($line =~ /^[ \t]*\\endinput/) {
			$line =~ s/(\\endinput.*)\n/% $1/;
			$in_comment = 1;
			process_line($line, $prefix, \$commented_newline);
			last;
		}
		process_line($line, $prefix, \$commented_newline, $file);
		if ($line =~ /^%.*[^\n]\z/ || $line =~ /[^\\]%.*[^\n]\z/) {
			# file ends with a comment not ending with a newline
			print "\n";
		}
		# Garbage at end of line after \end{document} is
		# ignored by LaTeX, but we don't allow anything before
		# to avoid e.g. \verb|\end{document}| from terminating
		# the file.
		if (!$keep_comments && $line =~ /^[ \t]*\\end\{document\}/) {
			last;
		}
	}
	close($FILE);
	return $in_comment;
}

sub process_line
{
	my ($line, $prefix, $commented_newline, $file) = @_;
	$_ = $line;
	if ($$commented_newline) {
		# Leading whitespaces after a comment is ignored.
		# There's no space in:
		# Line 1%
		#    Line 2.
		# Match just space and tabs (\s would match \n)
		s/^[ \t]*//;
		if (/^$/) {
			# Deal with:
			#
			# Line 1 % comment
			#
			# Line 2
			#
			# The newline after Line 1 is commented, but we still
			# want a new paragraph. We strip the comment together
			# with its newline, but re-add a newline to chnge
			# paragraph here if needed:
			print "\n";
		}
	}
	$$commented_newline = 0;
	# Consider \makeatletter only in preamble, because we do want
	# to warn on \someCommand{\makeatletter\command@with@arobase}.
	if ($in_preamble && /^[^%]*\\makeatletter/) {
		$makeatletter_found = 1;
	}
	if ($in_preamble && /^[^%]*\\makeatother/) {
		$makeatletter_found = 0;
	}
	my $command;
	if (!$makeatletter && !$makeatletter_found
	    && (($command) = /^[^%]*(\\[[:alpha:]]*@[[:alpha:]]*)/)
	    && ($command ne '\@')) {
		print STDERR "Warning: command $command containing @ found in\n";
		print STDERR "Warning: $file.\n";
		print STDERR "Warning: consider using --makeatletter if the result is not compilable.\n";
	}

        # non-comment is a sequence of:
        # - escaped character (\\.), including \% and \\
        # - neither '%' nor '\'.
        my $NON_COMMENT = '([^\\\\%]|\\\\.)*';

	unless ($keep_comments) {
		if (!$empty_comments) {
			# Include \n in pattern to avoid matching
			# comments at end of files

			# remove comments + whitespace-only lines completely
			if (s/^\s*%.*\n//) {
				$$commented_newline = 1;
			}

			# Special-case commands at end of line. We
			# don't want "\\foo%\nbar" to become
			# "\\foobar"
			if (s/^($NON_COMMENT\\[[:alpha:]@]+)%.*\n/$1 /) {
				$$commented_newline = 1;
			} elsif (s/^($NON_COMMENT)%.*\n/$1/) {
				# remove only the comment if the line has actual content
				$$commented_newline = 1;
			}
		}
		# Apply the "empty comments" treatment unconditionally
		# for comments not matched above (it doesn't harm to
		# keep an empty comment sometimes, but it may harm to
		# leave a real comment if the goal was to strip them).
		s/^(([^\\%]|\\.)*)%.*$/$1%/;
	}

	unless ($keep_includes) {
		# \input{foo.tex}
		my $ARGBRACES = '\{\\s*([^"}\\s][^}]*)(\\s*)\}';
		# \input{"foo bar.tex"}
		my $ARGQUOTED = '\{\\s*"([^"]*)"(\\s*)\}';
		# \input foo.tex
		my $ARGSPACES = '\\s([^\{\\s][^\\s]+?)\\s()';
		my $ARGUMENT = "\\s*?(?|$ARGBRACES|$ARGQUOTED|$ARGSPACES)";

		if (my ($before, $ignored, $full_filename, $trailing, $after)
		    = /^($NON_COMMENT)\\include$ARGUMENT(.*)$/) {
			$full_filename = find_tex_file($full_filename . ".tex");
			if ($full_filename) {
				say $prefix . "Found include for file: $full_filename\n";
				print $before . $nl;
				print '\clearpage{}' . $nl;
				print "% start include $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end include $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				print '\clearpage{}' . $nl;
				print $nl . $after . "\n";
				$_ = "";
			}
		} elsif (my ($before, $ignored, $full_filename, $trailing,  $after)
			 = /^($NON_COMMENT)\\input$ARGUMENT(.*)$/) {
                        if ($inside_import) {
                              $full_filename = $inside_import . $full_filename;
                        }
			$full_filename = find_tex_file($full_filename, ":.tex");
			if ($full_filename) {
				say $prefix . "Found input for file: $full_filename\n";
				# Surprisingly, space after filename
				# in \input{foo.tex } is inserted
				# _before_ the inclusion. Apply this
				# rule in latexpand.
				print $before . $trailing . $nl;
				print "% start input $full_filename\n" if ($explain);
				my $in_comment = process_file($full_filename, $prefix . "  ");
				if ($explain) {
				    print " % end input $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				if ($after =~ /[^\s]/) {
				    # LaTeX produces this space, so let's do it also
				    print " " . $nl . $after . "\n";
				} else {
				    print " ";
				}
				$_ = "";
			}
		} elsif (my ($before, $ignored, $dir, $ignored, $full_filename, $ignored,  $after)
			 = /^($NON_COMMENT)\\(?:sub)?import$ARGUMENT$ARGUMENT(.*)$/) {
                        if ($explain) {
                              print "% dir " . $dir ."\n";
                              print "% full_filename " . $full_filename ."\n";
                              print "% after " . $after ."\n";
                              print "% inside_import $inside_import\n";
                        }
                        $full_filename = $dir . $full_filename;
                        if ($inside_import) {
                              $full_filename = $inside_import . $full_filename;
                        }
                        print "% cat(inside_import,dir,full_filename) " . $full_filename ."\n" if ($explain);
			$full_filename = find_tex_file($full_filename, ":.tex");
			if ($full_filename) {
				say $prefix . "Found input for file: $full_filename\n";
				print $before . $nl;
				print "% start input $full_filename\n" if ($explain);
                                my $previous_import_dir = $inside_import;
                                $inside_import = $inside_import . $dir;
				my $in_comment = process_file($full_filename, $prefix . "  ");
                                $inside_import = $previous_import_dir;
				if ($explain) {
				    print " % end input $full_filename\n";
				} elsif ($in_comment) {
				    print "\n";
				}
				if ($after =~ /[^\s]/) {
				    # LaTeX produces this space, so let's do it also
				    print " " . $nl . $after . "\n";
				} else {
				    print " ";
				}
				$_ = "";
			}
		} elsif (my ($before, $ignored, $args, $full_filename, $ignored, $after)
			 = /^($NON_COMMENT)\\includegraphics[\[\s]+(.*?)[\s\]]$ARGUMENT(.*)$/) {
                        if ($explain) {
                                print "% inside_import " . $inside_import ."\n";
                                print "% before " . $before ."\n";
                                print "% ignored " . $ignored ."\n";
                                print "% args " . $args ."\n";
                                print "% full_filename " . $full_filename ."\n";
                                print "% after " . $after ."\n";
                        }
                        if ($inside_import) {
                                $full_filename = $inside_import . $full_filename;
                                print "$before\\includegraphics[$args]{$full_filename}$after\n";
                                $_ = "";
                        }
		} elsif (my ($before, $ignored, $args, $full_filename, $ignored, $after)
			 = /^($NON_COMMENT)\\lstinputlisting[\[\s]+(.*?)[\s\]]$ARGUMENT(.*)$/) {
                        if ($explain) {
                                print "% inside_import " . $inside_import ."\n";
                                print "% before " . $before ."\n";
                                print "% ignored " . $ignored ."\n";
                                print "% args " . $args ."\n";
                                print "% full_filename " . $full_filename ."\n";
                                print "% after " . $after ."\n";
                        }
                        if ($inside_import) {
                                $full_filename = $inside_import . $full_filename;
                                print "$before\\lstinputlisting[$args]{$full_filename}$after\n";
                                $_ = "";
                        }
		}
	}
	if ($expand_usepackage) {
		# Don't bother with before and after text, we just require the
		# usepackage to be alone on its line.
		if (my ($package_name) = /^\s*\\usepackage\{([^\}]*)\}\s*(%.*)?$/) {
			my $full = find_file($package_name . ".sty", $TEXINPUTS);
			if ($full) {
				say $prefix . "Found package file: $full\n";
				process_file($full, $prefix . "  ");
				$_ = "";
				# Forget about any commented newline
				# before the \usepackage:
				$$commented_newline = 0;
			} else {
				say $prefix . "Not including external package $package_name\n";
			}
		}
	}
	if ($expand_bbl) {
		if (my ($before, $bib_name, $after)
			 = /^(.*)\\(?:bibliography|bibselect)\{([^\}]*)\}(.*)$/) {
			# The BBL file is not necessarily $bib_name.
			# Take it from the command-line.
			print $before . $nl;
			say $prefix . "Expanding BBL file: $expand_bbl\n";
			process_file($expand_bbl, $prefix . "  ");
			print " " . $nl . $after . "\n";
			$_ = "";
		}
	}
	if ($biber) {
		if (my ($before, $after)
		    = /^(.*)\\(?:addbibresource)\{[^\}]*\}(.*)$/) {
			# See https://tex.stackexchange.com/questions/166518/biblatex-include-bbl-problem-with-verb-field/166526#166526
			my $biber_noext = $biber;
			$biber_noext =~ s/.bbl//;
			print $before . $nl;
			say $prefix . "Expanding Biber BBL file: $biber\n";
			print '\begin{filecontents*}{' . $biber . '}' . "\n";
			cat_file($biber);
			print "\n";
			print '\end{filecontents*}

\usepackage{xpatch}

%Patch the biblatex input command.
%replace "testinput-bbl" if you change the name above.
%disable if you want to run biblatex/biber normally
\makeatletter
\patchcmd\blx@bblinput{\blx@blxinit}
                      {\blx@blxinit
                       \def\jobname{' . $biber_noext . '}%new jobname
                      }{}{\fail}
\makeatother
			    ';
			say $prefix . "End expansion of Biber BBL file: $biber\n";
			print " " . $nl . $after . "\n";
			$_ = "";
		}
	}
	if ($show_graphics) {
		if (/\\includegraphics(\[[^\]]*\])?{([^}]*)}/) {
                        my $full_filename = $2;
                        if ($inside_import) {
                                $full_filename = $inside_import . $full_filename;
                        }
			my $full = find_tex_file($full_filename, $graphics_extensions);
			say $prefix . "needs graphics file: ";
			print STDERR "$full\n";
		}
	}
	if (/^[ \t]*\\begin\{document\}/) {
		$in_preamble = 0;
		if ($makeatletter) {
			print '\makeatletter' . $nl;
		}
	}
	print;
}

sub unquote
{
	my $str = shift;
	my $x = substr($str, 0, 1);
	my $y = substr($str, -1, 1);
	if ($x eq $y && ($x eq '"' || $x eq "'")) {
		$str = substr($str, 1, -1);
	}
	# There's a weird LaTeX syntax: \include{"file\space
	# with\space spaces"}, so remove these \space when unquoting.
	$str =~ s/\\space / /g;
	return $str;
}

# search $1 in $TEXINPUTS, with possible extensions in $2
sub find_tex_file
{
	my $file = unquote(shift);
	my $extensions = (shift || ":");
	foreach my $ext (split(':', $extensions, -1)) {
		my $full = find_file_global($file . $ext);
		if ($full) {
			return $full;
		}
	}
	if ($fatal) {
		die "ERROR: Could not find file [$file]\n";
	} else {
		print STDERR "Warning: Could not find file [$file]\n";
		return;
	}
}

sub find_file_global
{
	my $file = shift;
	if (open(my $fh, "-|", "kpsewhich", $file)) {
		my $full = <$fh>;
		$full =~ s/\s+$//;
		close($fh);
		if ($full) {
			return $full;
		}
	}
	# Should be useless, but fall-back in case kpsewhich fails (or is not installed, or ...):
	return find_file($file, $TEXINPUTS);
}

# Find files, not searching for global files (to allow not expanding global .sty packages)
sub find_file
{
	my ($file, $path) = @_;
	if (File::Spec->file_name_is_absolute($file)) {
		if (-e "$file" && ! -d "$file") {
			return $file;
		} else {
			return;
		}
	}

	# TEXINPUTS=...: (trailing :) means "append default search
	# directories". We don't want global directories here, but
	# still add . that may be needed.
	if (substr($path, -1) eq ':') {
		$path .= '.';
	}
	foreach my $dir (split(':', $path)) {
		if (-e "$dir/$file" && ! -d "$dir/$file") {
			return("$dir/$file");
		}
	}
	return;
}


__END__

=head1 NAME

latexpand - Flatten LaTeX file by expanding \include and \input, ... and  remove comments

=head1 SYNOPSIS

latexpand [options] FILE...

=head2 Options:

	--verbose        show what's going on
	--keep-comments  don't strip comments (comments are lines
                         starting with %, and anything below
                         \end{document})
	--empty-comments keep empty comments (i.e. % at end of lines) for clarity
	--keep-includes  don't expand \input and \include directives
	--expand-usepackage
	                 Expand \usepackage{...} directives if the
	                 corresponding .sty file is found in
	                 $TEXINPUTS (or the current directory if
	                 $TEXINPUTS is not set)
	--expand-bbl FILE
	                 Expand the bibliography by inlining FILE
	                 (should be a *.bbl file)
	--biber FILE	 Include \bibliography{} with FILE's content,
	                 as needed by biblatex with the biber backend.
	                 (similar to --expand-bbl FILE, but for
	                 biber+biblatex).
	--help           this help message
	--output <file>, -o <file>
	                 generate output in <file>
	--explain        generate explanatory comments in output
	--show-graphics  show included graphics
	--graphics_extensions
	                 colon-separated list of possible graphics extensions
	                 (used by --show-graphics to find the actual graphics files)
	--fatal          Die in case a file can't be found.
	--makeatletter   Insert a \makeatletter in the preamble. In some
	                 rare cases it may break your document, but it
	                 may help fixing bad interactions between
	                 @-commands and inclusion (see BUGS section).
	--in-encoding FMT, --out-encoding FMT
			 File encoding used by input and output files.
			 This uses the same syntax as PerlIO's layers.
			 Example:
			 --in-encoding 'encoding(UTF-8)'
			 The default is 'bytes' and should always work.

=head1 USES

The most common use of latexpand is to simplify distribution of source
LaTeX files, typically to satisfy the requirement of editors and
archival sites (springer, arXiv.org, ...) who force the authors to
submit sources. One does not necessarily want to submit sources with
comments, and uploading a document made of several files including
each other is a bit painful. By default, latexpand answers both
problems by outputing a single LaTeX file that contain no comment.

=head1 GETTING LATEXPAND

The latest version of latexpand is available here:

  https://gitlab.com/latexpand/latexpand

Versions are uploaded to ctan.org from time to time:

  http://www.ctan.org/pkg/latexpand

=head1 BUGS

Please, report bugs on the issue tracker on the project site:

  https://gitlab.com/latexpand/latexpand/issues

=head2 Known bugs

=head3 Verbatim

latexpand currently ignores \begin{verbatim} ... \end{verbatim}, and
will therefore process any \include, \input, ... directives that
appear within verbatim environments (while it shouldn't).

LaTeX comments inside verbatim environments are also incorrectly
stripped. You can use --keep-comments as a workaround to avoid this.

=head3 Comment environment

It would be nice to remove code between \begin{comment} and
\end{comment} too if \usepackage{comment} is used.

Code like

	foo%
	\begin{comment}

will produce the incorrect

	foo\begin{comment}

A workaround is to use --empty-comments when such tricky usage of the
comments package is done.

=head3 \makeatletter and use with transfig/xfig with \scalebox{}

If \input{} or \include{} appears as argument to a command, and the
file included contains \makeatletter, then after expansion, the
\makeatletter and the @-command appear as argument to the command,
which is forbidden because the argument is parsed (and the @-command
badly tokenized) before being executed.

This happens with

	\scalebox{ \input{file-generated-by-xfig.pdf_t} }

Workaround: add \makeatletter before the scalebox manually in your
code, like

        \makeatletter{}
	\scalebox{ \input{file-generated-by-xfig.pdf_t} }
        \makeatother{}

In the case of xfig generated files, it is necessary only for the
first occurence.

A more brute-force workaround is to use latexpand --makeatletter.

=head1 SEE ALSO

Instructions to include only the relevant .bib items (french):

https://lacl.fr/~caubert/notes/portabilite-du-tex.html#dependances

=head1 VERSION

This is latexpand version v1.6.

